Robust and scalable h-adaptive aggregated unfitted finite elements for interface elliptic problems

This work introduces a novel, fully robust and highly-scalable, $h$-adaptive aggregated unfitted finite element method for large-scale interface elliptic problems. The new method is based on a recent distributed-memory implementation of the aggregated finite element method atop a highly-scalable Cartesian forest-of-trees mesh engine. It follows the classical approach of weakly coupling nonmatching discretisations at the interface to model internal discontinuities at the interface. We propose a natural extension of a single-domain parallel cell aggregation scheme to problems with a finite number of interfaces; it straightforwardly leads to aggregated finite element spaces that have the structure of a Cartesian product. We demonstrate, through standard numerical analysis and exhaustive numerical experimentation on several complex Poisson and linear elasticity benchmarks, that the new technique enjoys the following properties: well-posedness, robustness with respect to cut location and material contrast, optimal ($h$-adaptive) approximation properties, high scalability and easy implementation in large-scale finite element codes. As a result, the method offers great potential as a useful finite element solver for large-scale interface problems modelled by partial differential equations.

==> figures/run_a0b0c0d0e0f0g0_n1_l2_trace.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8640.00,8640.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1029,935){\makebox(0,0){\strut{}\LARGE{$-6$}}}%
      \csname LTb\endcsname%
      \put(2126,935){\makebox(0,0){\strut{}\LARGE{$-4$}}}%
      \csname LTb\endcsname%
      \put(3223,935){\makebox(0,0){\strut{}\LARGE{$-2$}}}%
      \csname LTb\endcsname%
      \put(4320,935){\makebox(0,0){\strut{}\LARGE{$0$}}}%
      \csname LTb\endcsname%
      \put(5417,935){\makebox(0,0){\strut{}\LARGE{$2$}}}%
      \csname LTb\endcsname%
      \put(6514,935){\makebox(0,0){\strut{}\LARGE{$4$}}}%
      \csname LTb\endcsname%
      \put(7611,935){\makebox(0,0){\strut{}\LARGE{$6$}}}%
      \csname LTb\endcsname%
      \put(4320,471){\makebox(0,0){\strut{}\LARGE{Material constrast: $\log_{10} \mu^+/\mu^-$}}}%
      \csname LTb\endcsname%
      \put(884,1200){\makebox(0,0)[r]{\strut{}\LARGE{$-1$}}}%
      \csname LTb\endcsname%
      \put(884,2807){\makebox(0,0)[r]{\strut{}\LARGE{$-0.5$}}}%
      \csname LTb\endcsname%
      \put(884,4413){\makebox(0,0)[r]{\strut{}\LARGE{$0$}}}%
      \csname LTb\endcsname%
      \put(884,6019){\makebox(0,0)[r]{\strut{}\LARGE{$0.5$}}}%
      \csname LTb\endcsname%
      \put(884,7626){\makebox(0,0)[r]{\strut{}\LARGE{$1$}}}%
      \csname LTb\endcsname%
      \put(69,4413){\rotatebox{-270}{\makebox(0,0){\strut{}\LARGE{Cube scaling: $a \to [0,1 + a h]^d$}}}}%
      \csname LTb\endcsname%
      \put(8395,346){\makebox(0,0)[l]{\strut{}\LARGE{$1.0\cdot10^{-1}$}}}%
      \csname LTb\endcsname%
      \put(8395,5529){\makebox(0,0)[l]{\strut{}\LARGE{$1.0\cdot10^{0}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{run_a0b0c0d0e0f0g0_n1_l2_trace-plot}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/run_a0b0c0d1e0f0g0_n1_l2_trace.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8640.00,8640.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1029,935){\makebox(0,0){\strut{}\LARGE{$-6$}}}%
      \csname LTb\endcsname%
      \put(2126,935){\makebox(0,0){\strut{}\LARGE{$-4$}}}%
      \csname LTb\endcsname%
      \put(3223,935){\makebox(0,0){\strut{}\LARGE{$-2$}}}%
      \csname LTb\endcsname%
      \put(4320,935){\makebox(0,0){\strut{}\LARGE{$0$}}}%
      \csname LTb\endcsname%
      \put(5417,935){\makebox(0,0){\strut{}\LARGE{$2$}}}%
      \csname LTb\endcsname%
      \put(6514,935){\makebox(0,0){\strut{}\LARGE{$4$}}}%
      \csname LTb\endcsname%
      \put(7611,935){\makebox(0,0){\strut{}\LARGE{$6$}}}%
      \csname LTb\endcsname%
      \put(4320,471){\makebox(0,0){\strut{}\LARGE{Material constrast: $\log_{10} \mu^+/\mu^-$}}}%
      \csname LTb\endcsname%
      \put(884,1200){\makebox(0,0)[r]{\strut{}\LARGE{$-1$}}}%
      \csname LTb\endcsname%
      \put(884,2807){\makebox(0,0)[r]{\strut{}\LARGE{$-0.5$}}}%
      \csname LTb\endcsname%
      \put(884,4413){\makebox(0,0)[r]{\strut{}\LARGE{$0$}}}%
      \csname LTb\endcsname%
      \put(884,6019){\makebox(0,0)[r]{\strut{}\LARGE{$0.5$}}}%
      \csname LTb\endcsname%
      \put(884,7626){\makebox(0,0)[r]{\strut{}\LARGE{$1$}}}%
      \csname LTb\endcsname%
      \put(69,4413){\rotatebox{-270}{\makebox(0,0){\strut{}\LARGE{Cube scaling: $a \to [0,1 + a h]^d$}}}}%
      \csname LTb\endcsname%
      \put(8395,346){\makebox(0,0)[l]{\strut{}\LARGE{$1.0\cdot10^{-2}$}}}%
      \csname LTb\endcsname%
      \put(8395,5529){\makebox(0,0)[l]{\strut{}\LARGE{$1.0\cdot10^{-1}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{run_a0b0c0d1e0f0g0_n1_l2_trace-plot}}%
    \gplfronttext
  \end{picture}%
\endgroup

